Orbital Facility Location Problem for Satellite Constellation Servicing Depots

This work proposes an adaptation of the Facility Location Problem for the optimal placement of on-orbit servicing depots for satellite constellations in high-altitude orbit. The high-altitude regime, such as Medium Earth Orbit (MEO), is a unique dynamical environment where existing low-thrust propulsion systems can provide the necessary thrust to conduct plane-change maneuvers between the various orbital planes of the constellation. As such, on-orbit servicing architectures involving servicer spacecraft that conduct round-trips between servicing depots and the client satellites of the constellation may be conceived. To this end, orbital facility location problem is a binary linear program, where the costs of operating and allocating the facility(ies) to satellites are considered in terms of the sum of Equivalent Mass to Low Earth Orbit (EMLEO), is proposed. The low-thrust transfers between the facilities and the clients are computed using a parallel implementation of a Lyapunov feedback controller. The total launch cost of the depot along with its servicers, propellant, and payload are taken into account as the cost to establish a given depot. The proposed approach is applied to designing on-orbit servicing depots for the Galileo and the GPS constellations.

==> backup_tex_files/OLD_results.tex <==
% =========================================================================== %
\section{Numerical Results}
\label{sec:numerical_results}
The proposed problem formulation is applied for a scenario servicing (1) the Quasi-Zenith Satellite System (QZSS), a geosynchronous orbit (GSO) constellation of Japanese satellite-based GPS augmentation system, and (2) the GPS constellation operated by the USA, located in medium Earth orbit (MEO). The Keplerian elements of the QZSS fleet and the GPS fleet are given in the Appendix. 
The launch vehicle, depot, and servicer specifications are given in Table \ref{tab:specs_lv_depot_servicer}. 
%
The problem is implemented in Julia and solved with Gurobi 9.1.0 \cite{gurobi}. 

% TABLE OF LV, DEPOT, MEV
\begin{table}[]
\centering
\caption{Launch Vehicle, depot, and servicer parameters}
\begin{tabular}{@{}ll|l|llll@{}}
\toprule
\multicolumn{2}{c|}{Launch Vehicle}                                                                                                & \multicolumn{1}{c|}{Depot}                                    & \multicolumn{4}{c}{Servicer}                                                                                                                              \\
\begin{tabular}[c]{@{}l@{}}Parking orbit\\ radius, km\end{tabular} & \begin{tabular}[c]{@{}l@{}}Specific\\ impulse, s\end{tabular} & \begin{tabular}[c]{@{}l@{}}Specific\\ impulse, s\end{tabular} & Max thrust, N & \begin{tabular}[c]{@{}l@{}}Specific\\ impulse, s\end{tabular} & Dry mass, kg & \begin{tabular}[c]{@{}l@{}}Payload\\ mass, kg\end{tabular} \\ \midrule
6573                                                               & 350                                                           & 250                                                           & 1.17          & 1790                                                          & 1500         & 1000                                                       \\ \bottomrule
\end{tabular}
\label{tab:specs_lv_depot_servicer}
\end{table}



% ------------------------------------------------------- %
\subsection{Servicing the Quasi-Zenith Satellite System Constellation}
%The orbital characteristics of the QZSS fleet is shown in Table \ref{tab:qzss_clients}. 
To date, 4 QZSS spacecraft are flying, and 3 additional satellites are planned to be added to the constellation. One of the four existing satellites is placed in a geostationary orbit (Satellite number 3), with an orbital plane that is vastly different from the other 3.
Hence, in this work, 6 spacecraft evenly spaced in RAAN at the orbital plane of the 3 existing GSO satellites nare considered. Table \ref{tab:qzs_facility_slots} shows the orbital slots considered for this problem. Note for this problem, the distance unit $\mathrm{DU} = 42164$ \SI{}{km}. For the QZSS servicing problem, $Y \in \mathbb{B}^{18360}$, and $X \in \mathbb{B}^{6 \times 18360}$, resulting in $128520$ variables. 

% TABLE OF ORBITAL SLOTS for QZSS
\begin{table}[]
\centering
\caption{Orbital slots considered for QZSS constellation servicing depot}
\begin{tabular}{@{}llr@{}}
\toprule
Element             & Slot(s)     & Number of slots \\
\midrule
Semi-major axis, DU             & 0.4:0.1:1.8 & 15   \\
Eccentricity                    & 0:0.05:0.8  & 17   \\
Inclination, \SI{}{deg}         & 43          & 1   \\
RAAN, \SI{}{deg}                & 0:30:330    & 12  \\
Argument of perigee, \SI{}{deg} & 0:60:300    & 6   \\
True anomaly, \SI{}{deg}        & 0           & 1   \\
\textit{Total}                  & -           & 18360 \\
\bottomrule
\end{tabular}
\label{tab:qzs_facility_slots}
\end{table}

Firstly, the problem is solved for a range of values of $\lambda$ and $\rho$. The resulting number of facilities and the total equivalent mass to LEO, calculated by the objective function \eqref{eq:oflp_prob_objective}, are shown in Figure \ref{fig:qzs_heatmap}. Interestingly, optimal solutions using 1 or 3 facilities were found for various combinations of $\lambda$ and $\rho$, but no solution with 2 facilities were found to be optimal. 
Focusing on the case where $\rho = 2$, the optimal solution with $\lambda = 2$ places 3 facilities, while the optimal solution for a larger $\lambda = 3$ places a single facility. 
Note that an increase in $\lambda$ may effectively be treated as an increase in dry mass of each facility. This is an insightful result where the trade-off between the amount to be launched to orbit against the propellant mass required to access all 6 satellites from a single facility has tipped off in favor of launching fewer facilities. 

Focusing on the column along $\rho = 2$, Figure \ref{fig:qzs_ae_dist} shows the distribution of $a$ and $e$ of the optimal facility(ies) for $\lambda$ between $1$ and $3$. In particular, for $\lambda=1$ and $\lambda=3$ the facilities have the same combinations of $a$ and $e$, but it is vastly different for $\lambda=3$, where the single facility is located in an orbit with $a$ above the constellation and a significantly higher eccentricity. While such an orbit would result in a higher launch cost, transfers involving significant plane changes from the facility to the client satellites would be more economical. 


% figure of heatmap
\begin{figure}
    \centering
    \includegraphics[width=0.99\linewidth]{Figs/qzs_heatmap.pdf}
    \caption{Number of facilities and total equivalent mass to LEO for varying $\lambda$ and $\rho$ for servicing QZSS constellation}
    \label{fig:qzs_heatmap} 
\end{figure}

% figure of a vs. e
\begin{figure}
    \centering
    \includegraphics[width=0.99\linewidth]{Figs/qzs_ae_dist.pdf}
    \caption{Facilities $a$ and $e$ for varying $\lambda$ with fixed $\rho = 2$  for servicing QZSS constellation}
    \label{fig:qzs_ae_dist} 
\end{figure}

% figure of satellites for lmb=2, rho=2
\begin{figure}
    \centering
    \includegraphics[width=0.98\linewidth]{Figs/qzs_faccomb_lmb2_rho2.pdf}
    \caption{QZSS constellation and corresponding facilities with $\lambda = 2$, $\rho = 2$}
    \label{fig:qzs_faccomb_lmb2_rho2}
\end{figure}


% % figure of orbits for QZS
% \begin{figure}
%     \centering
%     \includegraphics[width=0.9\linewidth]{Figs/qzs_orb_lmb2_rho4.pdf}
%     \caption{QZSS constellation and corresponding facilities with $\lambda = 2$, $\rho = 4$}
%     \label{fig:qzs_orb_lmb3_rho2}
% \end{figure}

% % figure of transfers
% \begin{figure}
%     \centering
%     \includegraphics[width=0.98\linewidth]{Figs/qzs_faccomb_lmb2_rho4.pdf}
%     \caption{Low-thrust transfers for servicing QZSS constellation with $\lambda = 2$, $\rho = 4$}
%     \label{fig:qzs_faccomb_lmb2_rho4}
% \end{figure}

% % figure of slots for QZS
% \begin{figure}
%     \centering
%     \includegraphics[width=0.85\linewidth]{Figs/qzs_slots_lmb2_rho4.pdf}
%     \caption{Orbital slots used by facilities for servicing QZSS constellation with $\lambda = 2$, $\rho = 4$}
%     \label{fig:qzs_slots_lmb2_rho4} 
%\end{figure}

% ------------------------------------------------------- %
\subsection{Servicing the GPS Constellation}
The orbital characteristics of the GPS fleet is shown in Table \ref{tab:gps_clients}. Compared to the QZSS constellation, the GPS constellation consists of a significantly larger 31 satellites, located on 6 orbital planes. It is also noted that at MEO, changes in orbital planes are more costly than at GSO. 
Table \ref{tab:gps_facility_slots} shows the orbital slots considered for this problem. Note for this problem, the distance unit $\mathrm{DU} = 26560$ \SI{}{km}. For the GPS servicing problem, $Y \in \mathbb{B}^{11088}$, and $X \in \mathbb{B}^{31 \times 11088}$, resulting in $354816$ variables.  

% TABLE OF ORBITAL SLOTS for GPS
\begin{table}[]
\centering
\caption{Orbital slots considered for GPS constellation servicing depot}
\begin{tabular}{@{}llr@{}}
\toprule
Element             & Slot(s)     & Number of slots \\
\midrule
Semi-major axis, DU             & 0.8:0.1:1.6 & 9   \\
Eccentricity                    & 0:0.04:0.3  & 8   \\
Inclination, \SI{}{deg}         & 55          & 1   \\
RAAN, \SI{}{deg}                & 0:30:330    & 12  \\
Argument of perigee, \SI{}{deg} & 0:60:300    & 6   \\
True anomaly, \SI{}{deg}        & 0           & 1   \\
\textit{Total}                  & -           & 11088 \\
\bottomrule
\end{tabular}
\label{tab:gps_facility_slots}
\end{table}

Figure \ref{fig:gps_heatmap} shows the solution to the problem for a range of values of $\lambda$ and $\rho$ for the GPS constellation.
Here again, as $\lambda$ increases, the number of facilities is observed to decrease, as visible for the cases where $\rho=1$ and $\rho=2$. Furthermore, for the chosen architecture parameters, no combination of $\lambda$ and $\rho$ led to an optimal solution with 4 facilities. 
Figure \ref{fig:gps_ae_dist} shows the distribution of $a$ and $e$ for optimal solutions with $\rho = 1$ and varying $\lambda$. 
Similarly to the case of the QZSS constellation, an increase in $\lambda$ does lead to less facilities located at orbital slots with larger $a$ and $e$, but it is found that the facilities are always located below the constellation itself, with $a < 1$ \SI{}{DU}. 
This is a consequence of the GPS constellation having a significantly larger number of satellites than the QZSS constellation; this makes servicing all members of the fleet with fewer facilities less advantageous than for the QZSS. Then, optimal solutions have the tendency to leverage more facilities at lower altitudes, where it is cheaper to deploy. 

% figure of heatmap
\begin{figure}
    \centering
    \includegraphics[width=0.99\linewidth]{Figs/gps_heatmap.pdf}
    \caption{Number of facilities and total equivalent mass to LEO for varying $\lambda$ and $\rho$  for servicing GPS constellation}
    \label{fig:gps_heatmap} 
\end{figure}

% figure of a vs. e
\begin{figure}
    \centering
    \includegraphics[width=0.99\linewidth]{Figs/gps_ae_dist.pdf}
    \caption{Facilities $a$ and $e$ for varying $\lambda$ with fixed $\rho = 1$  for servicing GPS constellation}
    \label{fig:gps_ae_dist} 
\end{figure}




==> backup_tex_files/table3_with_EMLEO.tex <==
% Table of CPLEX performance 
\begin{table}[]
    \centering
    \caption{CPLEX performance solving OFLP for GPS \& Galileo servicing facilities}
    \begin{tabular}{lllllllllll}
    \hline
    \hline
    %\begin{tabular}[c]{@{}l@{}} A, \\ B \end{tabular}
     & & \multicolumn{4}{c}{$D = 1$} &  & \multicolumn{4}{c}{$D = 2$}  
    \\
    \cline{3-6} \cline{8-10}
    \begin{tabular}[c]{@{}l@{}} $\msdry$, \\ \SI{}{kg} \end{tabular}
    & 
    \begin{tabular}[c]{@{}l@{}} $\mddry$, \\ \SI{}{kg} \end{tabular}
    & Status & 
    \begin{tabular}[c]{@{}l@{}} Objective, \\ \SI{}{kg} \end{tabular}
    & Gap & 
    \begin{tabular}[c]{@{}l@{}} Solve \\ time, \SI{}{sec}  \end{tabular}
    % -----------------------
    &  &   % EXTRA SPACE
    % -----------------------
    Status & 
    \begin{tabular}[c]{@{}l@{}} Objective, \\ \SI{}{kg} \end{tabular}
    & Gap & 
    \begin{tabular}[c]{@{}l@{}} Solve \\ time, \SI{}{sec}  \end{tabular}
    \\
    \hline
    \multirow{3}{*}{500}
    % D = 1                    /    D = 2
    & 1500 & OPTIMAL & 38079 & 0.0 & 655.929 & & OPTIMAL & 59833 & 0.0 & 174.511 \\
    & 2000 & OPTIMAL & 42294 & 0.0 & 155.637 & & OPTIMAL & 65431 & 0.0 & 119.195 \\
    & 2500 & OPTIMAL & 45287 & 0.0 & 156.419 & & OPTIMAL & 70865 & 0.0 & 133.745 \\
    \hline
    \multirow{3}{*}{1000}
    % D = 1                    /    D = 2
    & 1500 & OPTIMAL & 47019 & 0.0 & 295.819 & & OPTIMAL & 74732 & 0.0 & 257.044 \\
    & 2000 & OPTIMAL & 53192 & 0.0 & 461.123 & & OPTIMAL & 81195 & 0.0 & 281.117 \\
    & 2500 & OPTIMAL & 58786 & 0.0 & 787.712 & & OPTIMAL & 90427 & 0.0 & 2709.114 \\
    \hline
    \hline
    \end{tabular}
    \label{tab:cplex_solve_info}
\end{table}

==> backup_tex_files/table3_wo_EMLEO.tex <==
% Table of CPLEX performance 
\begin{table}[]
    \centering
    \caption{CPLEX performance solving OFLP for GPS \& Galileo servicing facilities}
    \begin{tabular}{lllllllll}
    \hline
    \hline
    %\begin{tabular}[c]{@{}l@{}} A, \\ B \end{tabular}
     & & \multicolumn{3}{c}{$D = 1$} &  & \multicolumn{3}{c}{$D = 2$}  
    \\
    \cline{3-5} \cline{7-9}
    \begin{tabular}[c]{@{}l@{}} $\msdry$, \\ \SI{}{kg} \end{tabular}
    & 
    \begin{tabular}[c]{@{}l@{}} $\mddry$, \\ \SI{}{kg} \end{tabular}
    & Status & 
    Gap & 
    \begin{tabular}[c]{@{}l@{}} Solve \\ time, \SI{}{sec}  \end{tabular}
    % -----------------------
    &  &   % EXTRA SPACE
    % -----------------------
    Status &  
    Gap & 
    \begin{tabular}[c]{@{}l@{}} Solve \\ time, \SI{}{sec}  \end{tabular}
    \\
    \hline
    \multirow{3}{*}{500}
    % D = 1                    /    D = 2
    & 1500 & OPTIMAL & 0.0 & 655.929 & & OPTIMAL & 0.0 & 174.511 \\
    & 2000 & OPTIMAL & 0.0 & 155.637 & & OPTIMAL & 0.0 & 119.195 \\
    & 2500 & OPTIMAL & 0.0 & 156.419 & & OPTIMAL & 0.0 & 133.745 \\
    \hline
    \multirow{3}{*}{1000}
    % D = 1                    /    D = 2
    & 1500 & OPTIMAL & 0.0 & 295.819 & & OPTIMAL & 0.0 & 257.044 \\
    & 2000 & OPTIMAL & 0.0 & 461.123 & & OPTIMAL & 0.0 & 281.117 \\
    & 2500 & OPTIMAL & 0.0 & 787.712 & & OPTIMAL & 0.0 & 2709.114 \\
    \hline
    \hline
    \end{tabular}
    \label{tab:cplex_solve_info}
\end{table}

==> backup_tex_files/table45_with_EMLEO.tex <==

% TABLE of GPS&GAL FACILITIES for 201
\begin{table}[]
\centering
\caption{Summary of optimal GPS \& Galileo servicing depots from OFLP instances with $\msdry = 500$ \SI{}{kg}}
\begin{tabular}{lllllllllllllllllll}
\hline
\hline
  & & \multicolumn{7}{c}{$D = 1$} &  & \multicolumn{7}{c}{$D = 2$}   \\
  \cline{3-10} \cline{12-19}
\begin{tabular}[c]{@{}l@{}} $\mddry$, \\ \SI{}{kg}  \end{tabular}
& No. & 
\begin{tabular}[c]{@{}l@{}} $a$, \\ \SI{}{DU} \end{tabular} &
%$a$, \SI{}{DU} &
$e$ & 
\begin{tabular}[c]{@{}l@{}} $i$,\\ \SI{}{deg} \end{tabular}  &
\begin{tabular}[c]{@{}l@{}} $\Omega$, \\ \SI{}{deg} \end{tabular}  &
$\mathcal{K}_a$  & 
\begin{tabular}[c]{@{}l@{}} $\mdwet$, \\ \SI{}{kg}  \end{tabular} &
\begin{tabular}[c]{@{}l@{}} EMLEO, \\ \SI{}{kg}  \end{tabular} &
\begin{tabular}[c]{@{}l@{}} Total \\ EMLEO, \SI{}{kg} \end{tabular} 
% -----------------------
&  &   % EXTRA SPACE
% -----------------------
\begin{tabular}[c]{@{}l@{}} $a$ \\ \SI{}{DU} \end{tabular} &
$e$ &
%$a$, \SI{}{DU} & 
\begin{tabular}[c]{@{}l@{}} $i$ \\ \SI{}{deg} \end{tabular}  &
\begin{tabular}[c]{@{}l@{}} $\Omega$ \\ \SI{}{deg} \end{tabular}  &
$\mathcal{K}_a$  & 
\begin{tabular}[c]{@{}l@{}} $\mdwet$ \\ \SI{}{kg}  \end{tabular} &
\begin{tabular}[c]{@{}l@{}} EMLEO \\ \SI{}{kg}  \end{tabular} &
\begin{tabular}[c]{@{}l@{}} Total \\ EMLEO, \SI{}{kg} \end{tabular} 
\\[0.8em]
\hline
% results for 1500
\multirow{6}{*}{1500} 
& 1 & 0.80 & 0.20 &  56 &  30 & 16 &  6015 &  9470  & \multirow{6}{*}{38,079} & & 0.95 & 0.10 &  55 &  30 & 16 &  9612 & 15416 & \multirow{6}{*}{59,833}\\
& 2 & 0.60 & 0.55 &  57 &  90 &  5 &  2758 &  4312 & & & 0.60 & 0.55 &  57 &  90 &  &  5 3973 &  6211 \\
& 3 & 0.60 & 0.55 &  55 & 150 & 14 &  4845 &  7575 & & & 0.60 & 0.55 &  55 & 150 & 14 &  8147 & 12737 \\
& 4 & 0.55 & 0.50 &  54 & 210 &  4 &  2501 &  3799 & & & 0.60 & 0.55 &  53 & 210 &  4 &  3343 &  5227 \\
& 5 & 0.60 & 0.55 &  57 & 270 & 13 &  4682 &  7320 & & & 0.60 & 0.55 &  57 & 270 & 13 &  7821 & 12226 \\
& 6 & 0.55 & 0.50 &  54 & 330 &  7 &  3688 &  5603 & & & 0.95 & 0.05 &  55 & 330 &  7 &  5048 &  8016 \\
\hline
% results for 2000
\multirow{6}{*}{2000} 
& 1 & 0.75 & 0.25 &  55 &  30 & 16 &  6734 & 10546 & \multirow{5}{*}{42,294} & & 0.90 & 0.10 &  55 &  30 & 16 & 10475 & 16606 & \multirow{6}{*}{65,431} \\
& 2 & 0.40 & 0.35 &  53 &  90 &  5 &  3726 &  5022 & & & 0.60 & 0.55 &  57 &  90 &  5 &  4487 &  7015 \\
& 3 & 0.60 & 0.55 &  55 & 150 & 14 &  5360 &  8379 & & & 0.60 & 0.55 &  55 & 150 & 14 &  8662 & 13541 \\
& 4 & 0.65 & 0.60 &  51 & 240 & 17 &  7473 & 11973 & & & 0.55 & 0.50 &  54 & 210 &  4 &  3963 &  6021 \\
& 5 & 0.50 & 0.45 &  53 & 330 &  7 &  4338 &  6374 & & & 0.60 & 0.55 &  57 & 270 & 13 &  8335 & 13031 \\
& 6 & \multicolumn{7}{c}{Unused}      & & & 0.90 & 0.10 &  54 & 330 &  7 &  5814 &  9216 \\
\hline
% results for 2500
\multirow{6}{*}{2500} 
& 1 & 0.90 & 0.55 &  53 &   0 & 23 & 10724 & 18172 & \multirow{3}{*}{45,287} & & 0.90 & 0.10 &  55 &  30 & 16 & 11215 & 17779 & \multirow{6}{*}{70,865} \\
& 2 & 0.65 & 0.60 &  52 & 120 & 19 &  8942 & 14328 & & & 0.60 & 0.55 &  57 &  90 &  5 &  5002 &  7819 \\
& 3 & 0.65 & 0.60 &  51 & 240 & 17 &  7980 & 12786 & & & 0.60 & 0.55 &  55 & 150 & 14 &  9176 & 14346 \\
& 4 &  \multicolumn{7}{c}{Unused}     & & & 0.55 & 0.50 &  54 & 210 &  4 &  4482 &  6810 \\
& 5 &  \multicolumn{7}{c}{Unused}     & & & 0.60 & 0.55 &  57 & 270 & 13 &  8850 & 13835 \\
& 6 &  \multicolumn{7}{c}{Unused}     & & & 0.65 & 0.25 &  54 & 330 &  7 &  6790 & 10276\\ 
\hline
\hline
\end{tabular}
\label{tab:used_elts_FLP_gpsgal_ms500}
\end{table}


% TABLE of GPS&GAL FACILITIES for 202
\begin{table}[]
\centering
\caption{Summary of optimal GPS \& Galileo servicing depots from OFLP instances with $\msdry = 1000$ \SI{}{kg}}
\begin{tabular}{lllllllllllllllllll}
\hline
\hline
  & & \multicolumn{7}{c}{$D = 1$} &  & \multicolumn{7}{c}{$D = 2$}   \\
  \cline{3-10} \cline{12-19}
\begin{tabular}[c]{@{}l@{}} $\mddry$, \\ \SI{}{kg}  \end{tabular}
& No. & 
\begin{tabular}[c]{@{}l@{}} $a$, \\ \SI{}{DU} \end{tabular} &
%$a$, \SI{}{DU} &
$e$ & 
\begin{tabular}[c]{@{}l@{}} $i$,\\ \SI{}{deg} \end{tabular}  &
\begin{tabular}[c]{@{}l@{}} $\Omega$, \\ \SI{}{deg} \end{tabular}  &
$\mathcal{K}_a$  & 
\begin{tabular}[c]{@{}l@{}} $\mdwet$, \\ \SI{}{kg}  \end{tabular} &
\begin{tabular}[c]{@{}l@{}} EMLEO, \\ \SI{}{kg}  \end{tabular} &
\begin{tabular}[c]{@{}l@{}} Total \\ EMLEO, \SI{}{kg} \end{tabular} 
% -----------------------
&  &   % EXTRA SPACE
% -----------------------
\begin{tabular}[c]{@{}l@{}} $a$ \\ \SI{}{DU} \end{tabular} &
$e$ &
%$a$, \SI{}{DU} & 
\begin{tabular}[c]{@{}l@{}} $i$ \\ \SI{}{deg} \end{tabular}  &
\begin{tabular}[c]{@{}l@{}} $\Omega$ \\ \SI{}{deg} \end{tabular}  &
$\mathcal{K}_a$  & 
\begin{tabular}[c]{@{}l@{}} $\mdwet$ \\ \SI{}{kg}  \end{tabular} &
\begin{tabular}[c]{@{}l@{}} EMLEO \\ \SI{}{kg}  \end{tabular} &
\begin{tabular}[c]{@{}l@{}} Total \\ EMLEO, \SI{}{kg} \end{tabular} 
\\[0.8em]
\hline
% results for 1500
\multirow{6}{*}{1500} 
& 1 & 1.00 & 0.10 &  55 &  30 & 16 &  7028 & 11392 & \multirow{6}{*}{47,019} & & 1.00 & 0.10 &  55 &  30 & 16 & 11811 & 19146 & \multirow{6}{*}{74,732} \\
& 2 & 0.60 & 0.55 &  58 &  90 &  5 &  3377 &  5279 & & & 0.60 & 0.55 &  58 &  90 &  5 &  5211 &  8146 \\
& 3 & 0.95 & 0.10 &  55 & 150 & 14 &  6208 &  9956 & & & 0.95 & 0.10 &  55 & 150 & 14 & 10183 & 16331 \\
& 4 & 0.60 & 0.55 &  53 & 210 &  4 &  2886 &  4513 & & & 0.60 & 0.55 &  53 & 210 &  4 &  4230 &  6612 \\
& 5 & 0.95 & 0.15 &  55 & 270 & 13 &  5936 &  9609 & & & 1.00 & 0.10 &  55 & 270 & 13 &  9659 & 15658 \\
& 6 & 0.95 & 0.05 &  55 & 330 &  7 &  3948 &  6270 & & & 1.00 & 0.00 &  56 & 330 &  7 &  5564 &  8839 \\
\hline
% results for 2000
\multirow{6}{*}{2000} 
& 1 & 0.95 & 0.10 &  55 &  30 & 16 &  7849 & 12589 & \multirow{6}{*}{53,192} & & 1.00 & 0.10 &  55 &  30 & 16 & 12559 & 20358  & \multirow{6}{*}{81,195}
\\
& 2 & 0.60 & 0.55 &  58 &  90 &  5 &  3891 &  6084 & & & 0.60 & 0.55 &  58 &  90 &  5 &  5725 &  8950 
\\
& 3 & 0.60 & 0.55 &  55 & 150 & 14 &  7061 & 11038 & & & 0.95 & 0.10 &  55 & 150 & 14 & 10927 & 17525 
\\
& 4 & 0.55 & 0.50 &  54 & 210 &  4 &  3498 &  5315  & & & 0.60 & 0.55 &  53 & 210 &  4 &  4744 &  7416 
\\
& 5 & 0.60 & 0.55 &  56 & 270 & 13 &  6833 & 10682 & & & 0.95 & 0.10 &  55 & 270 & 13  & 10507 & 16852 
\\
& 6 & 0.95 & 0.05 &  55 & 330 &  7 &  4713 &  7484  & & & 1.00 & 0.00 &  56 & 330 &  7  &  6353 & 10093 
\\
\hline
% results for 2500
\multirow{6}{*}{2500} 
& 1 & 0.95 & 0.10 &  55 &  30 & 16 &  8594 & 13783  & \multirow{6}{*}{58,786} & & 1.00 & 0.10 &  55 &  30 & 15 & 12653 & 20510  & \multirow{6}{*}{90,427} \\
& 2 & 0.60 & 0.55 &  58 &  90 &  5 &  4406 &  6888 & & & 0.60 & 0.55 &  58 &  90 &  5 &  6240 &  9754  \\
& 3 & 0.60 & 0.55 &  55 & 150 & 14 &  7575 & 11842  & & & 0.95 & 0.10 &  55 & 150 & 14 & 11671 & 18719  \\
& 4 & 0.55 & 0.50 &  54 & 210 &  4 &  4018 &  6104  & & & 0.60 & 0.55 &  53 & 210 &  4 &  5258 &  8221  \\
& 5 & 0.60 & 0.55 &  56 & 270 & 13 &  7348 & 11487  & & & 0.95 & 0.10 &  55 & 270 & 13 & 11252 & 18046 \\
& 6 & 0.90 & 0.10 &  55 & 330 &  7 &  5477 &  8682  & & & 1.00 & 0.05 &  56 & 330 &  8 &  9453 & 15176  \\ 
\hline
\hline
\end{tabular}
\label{tab:used_elts_FLP_gpsgal_ms1000}
\end{table}

==> backup_tex_files/table45_wo_EMLEO.tex <==
% TABLE of GPS&GAL FACILITIES for 201
\begin{table}[]
\centering
\caption{Summary of optimal GPS \& Galileo servicing depots from OFLP instances with $\msdry = 500$ \SI{}{kg}}
\begin{tabular}{lllllllllllllll}
\hline
\hline
%\begin{tabular}[c]{@{}l@{}} A, \\ B \end{tabular}
  & & \multicolumn{6}{c}{$D = 1$} &  & \multicolumn{6}{c}{$D = 2$}   \\
  \cline{3-8} \cline{10-15}
\begin{tabular}[c]{@{}l@{}} $\mddry$ \\ \SI{}{kg}  \end{tabular}
& No. & 
\begin{tabular}[c]{@{}l@{}} $a$ \\ \SI{}{DU} \end{tabular} &
%$a$, \SI{}{DU} &
$e$ & 
\begin{tabular}[c]{@{}l@{}} $i$ \\ \SI{}{deg} \end{tabular}  &
%$i$, \SI{}{deg} & 
\begin{tabular}[c]{@{}l@{}} $\Omega$ \\ \SI{}{deg} \end{tabular}  &
%$\Omega$, \SI{}{deg}  &
\begin{tabular}[c]{@{}l@{}} $\mdwet$ \\ \SI{}{kg}  \end{tabular} &
%\begin{tabular}[c]{@{}l@{}} EMLEO \\ \SI{}{kg}  \end{tabular} &
%$\mdwet$, \SI{}{kg} 
$\mathcal{K}_a$ 
% -----------------------
&  &   % EXTRA SPACE
% -----------------------
\begin{tabular}[c]{@{}l@{}} $a$ \\ \SI{}{DU} \end{tabular} &
$e$ &
%$a$, \SI{}{DU} & 
\begin{tabular}[c]{@{}l@{}} $i$ \\ \SI{}{deg} \end{tabular}  &
%$i$, \SI{}{deg} & 
\begin{tabular}[c]{@{}l@{}} $\Omega$ \\ \SI{}{deg} \end{tabular}  &
%$\Omega$, \SI{}{deg}  &
\begin{tabular}[c]{@{}l@{}} $\mdwet$ \\ \SI{}{kg}  \end{tabular} &
%\begin{tabular}[c]{@{}l@{}} EMLEO \\ \SI{}{kg}  \end{tabular} &
%$\mdwet$, \SI{}{kg} & 
$\mathcal{K}_a$  
\\[0.8em]
\hline
% results for 1500
\multirow{6}{*}{1500} & 1 & 0.80 & 0.20 &  56 &  30 &  6015  & 16 & & 0.95 & 0.10 &  55 &  30 &  9612 & 16 \\
                      & 2 & 0.60 & 0.55 &  57 &  90 &  2758  &  5 & & 0.60 & 0.55 &  57 &  90 &  3973 &  5 \\
                      & 3 & 0.60 & 0.55 &  55 & 150 &  4845 & 14 & & 0.60 & 0.55 &  55 & 150 &  8147 & 14 \\
                      & 4 & 0.55 & 0.50 &  54 & 210 &  2501 &  4 & & 0.60 & 0.55 &  53 & 210 &  3343 &  4 \\
                      & 5 & 0.60 & 0.55 &  57 & 270 &  4682 & 13 & & 0.60 & 0.55 &  57 & 270 &  7821 & 13 \\
                      & 6 & 0.55 & 0.50 &  54 & 330 &  3688 &  7 & & 0.95 & 0.05 &  55 & 330 &  5048 &  7 \\
\hline
% results for 2000
\multirow{6}{*}{2000} & 1 & 0.75 & 0.25 &  55 &  30 &  6734 & 16 & & 0.90 & 0.10 &  55 &  30 & 10475 & 16 \\
                      & 2 & 0.40 & 0.35 &  53 &  90 &  3726 &  5 & & 0.60 & 0.55 &  57 &  90 &  4487 &  5 \\
                      & 3 & 0.60 & 0.55 &  55 & 150 &  5360 & 14 & & 0.60 & 0.55 &  55 & 150 &  8662 & 14 \\
                      & 4 & 0.65 & 0.60 &  51 & 240 &  7473 & 17 & & 0.55 & 0.50 &  54 & 210 &  3963 &  4 \\
                      & 5 & 0.50 & 0.45 &  53 & 330 &  4338 &  7 & & 0.60 & 0.55 &  57 & 270 &  8335 & 13 \\
                      & 6 & \multicolumn{6}{c}{Unused}       & & 0.90 & 0.10 &  54 & 330 &  5814 &  7 \\
\hline
% results for 2500
\multirow{6}{*}{2500} & 1 & 0.90 & 0.55 &  53 &   0 & 10724 & 23 & & 0.90 & 0.10 &  55 &  30 & 11215 & 16  \\
                      & 2 & 0.65 & 0.60 &  52 & 120 &  8942 & 19 & & 0.60 & 0.55 &  57 &  90 &  5002 &  5 \\
                      & 3 & 0.65 & 0.60 &  51 & 240 &  7980 & 17 & & 0.60 & 0.55 &  55 & 150 &  9176 & 14 \\
                      & 4 &  \multicolumn{6}{c}{Unused}     & & 0.55 & 0.50 &  54 & 210 &  4482 &  4 \\
                      & 5 &  \multicolumn{6}{c}{Unused}     & & 0.60 & 0.55 &  57 & 270 &  8850 & 13 \\
                      & 6 &  \multicolumn{6}{c}{Unused}     & & 0.65 & 0.25 &  54 & 330 &  6790 &  7 \\ 
\hline
\hline
\end{tabular}
\label{tab:used_elts_FLP_gpsgal_ms500}
\end{table}


% TABLE of GPS&GAL FACILITIES for 202
\begin{table}[]
\centering
\caption{Summary of optimal GPS \& Galileo servicing depots from OFLP instances with $\msdry = 1000$ \SI{}{kg}}
\begin{tabular}{lllllllllllllll}
\hline
\hline
%\begin{tabular}[c]{@{}l@{}} A, \\ B \end{tabular}
  & & \multicolumn{6}{c}{$D = 1$} &  & \multicolumn{6}{c}{$D = 2$}   \\
  \cline{3-8} \cline{10-15}
  % & & \multicolumn{7}{c}{$D = 1$} &  & \multicolumn{7}{c}{$D = 2$}   \\
  % \cline{3-9} \cline{11-17}
\begin{tabular}[c]{@{}l@{}} $\mddry$ \\ \SI{}{kg}  \end{tabular}
& No. & 
\begin{tabular}[c]{@{}l@{}} $a$ \\ \SI{}{DU} \end{tabular} &
%$a$, \SI{}{DU} &
$e$ & 
\begin{tabular}[c]{@{}l@{}} $i$ \\ \SI{}{deg} \end{tabular}  &
%$i$, \SI{}{deg} & 
\begin{tabular}[c]{@{}l@{}} $\Omega$ \\ \SI{}{deg} \end{tabular}  &
%$\Omega$, \SI{}{deg}  &
\begin{tabular}[c]{@{}l@{}} $\mdwet$ \\ \SI{}{kg}  \end{tabular} &
%\begin{tabular}[c]{@{}l@{}} EMLEO \\ \SI{}{kg}  \end{tabular} &
%$\mdwet$, \SI{}{kg} 
$\mathcal{K}_a$ 
% -----------------------
&  &   % EXTRA SPACE
% -----------------------
\begin{tabular}[c]{@{}l@{}} $a$ \\ \SI{}{DU} \end{tabular} &
$e$ &
%$a$, \SI{}{DU} & 
\begin{tabular}[c]{@{}l@{}} $i$ \\ \SI{}{deg} \end{tabular}  &
%$i$, \SI{}{deg} & 
\begin{tabular}[c]{@{}l@{}} $\Omega$ \\ \SI{}{deg} \end{tabular}  &
%$\Omega$, \SI{}{deg}  &
\begin{tabular}[c]{@{}l@{}} $\mdwet$ \\ \SI{}{kg}  \end{tabular} &
%\begin{tabular}[c]{@{}l@{}} EMLEO \\ \SI{}{kg}  \end{tabular} &
%$\mdwet$, \SI{}{kg} & 
$\mathcal{K}_a$ 
\\[0.8em]
\hline
% results for 1500
\multirow{6}{*}{1500} & 1 & 1.00 & 0.10 &  55 &  30 &  7028 & 16 & & 1.00 & 0.10 &  55 &  30 & 11811 & 16 \\
                      & 2 & 0.60 & 0.55 &  58 &  90 &  3377 &  5 & & 0.60 & 0.55 &  58 &  90 &  5211 &  5 \\
                      & 3 & 0.95 & 0.10 &  55 & 150 &  6208 &  14 & & 0.95 & 0.10 &  55 & 150 & 10183 & 14 \\
                      & 4 & 0.60 & 0.55 &  53 & 210 &  2886 &    4 & & 0.60 & 0.55 &  53 & 210 &  4230 &  4 \\
                      & 5 & 0.95 & 0.15 &  55 & 270 &  5936 &  13 & & 1.00 & 0.10 &  55 & 270 &  9659 & 13 \\
                      & 6 & 0.95 & 0.05 &  55 & 330 &  3948 &   7 & & 1.00 & 0.00 &  56 & 330 &  5564 &  7 \\
\hline
% results for 2000
\multirow{6}{*}{2000} & 1 & 0.95 & 0.10 &  55 &  30 &  7849 & 16 & & 1.00 & 0.10 &  55 &  30 & 12559 & 16 \\
                      & 2 & 0.60 & 0.55 &  58 &  90 &  3891 &  5 & & 0.60 & 0.55 &  58 &  90 &  5725 &  5 \\
                      & 3 & 0.60 & 0.55 &  55 & 150 &  7061 & 14 & & 0.95 & 0.10 &  55 & 150 & 10927 & 14 \\
                      & 4 & 0.55 & 0.50 &  54 & 210 &  3498 &  4 & & 0.60 & 0.55 &  53 & 210 &  4744 &  4\\
                      & 5 & 0.60 & 0.55 &  56 & 270 &  6833 & 13 & & 0.95 & 0.10 &  55 & 270 & 10507 & 13 \\
                      & 6 & 0.95 & 0.05 &  55 & 330 &  4713 &  7 & & 1.00 & 0.00 &  56 & 330 &  6353 &  7 \\
\hline
% results for 2500
\multirow{6}{*}{2500} & 1 & 0.95 & 0.10 &  55 &  30 &  8594 & 16 & & 1.00 & 0.10 &  55 &  30 & 12653 & 15 \\
                      & 2 & 0.60 & 0.55 &  58 &  90 &  4406 &  5 & & 0.60 & 0.55 &  58 &  90 &  6240 &  5 \\
                      & 3 & 0.60 & 0.55 &  55 & 150 &  7575 & 14 & & 0.95 & 0.10 &  55 & 150 & 11671 & 14 \\
                      & 4 & 0.55 & 0.50 &  54 & 210 &  4018 &  4 & & 0.60 & 0.55 &  53 & 210 &  5258 &  4 \\
                      & 5 & 0.60 & 0.55 &  56 & 270 &  7348 & 13 & & 0.95 & 0.10 &  55 & 270 & 11252 & 13 \\
                      & 6 & 0.90 & 0.10 &  55 & 330 &  5477 &  7 & & 1.00 & 0.05 &  56 & 330 &  9453 &  8 \\ 
\hline
\hline
\end{tabular}
\label{tab:used_elts_FLP_gpsgal_ms1000}
\end{table}


==> backup_tex_files/table6_before_modification.tex <==

% Refined facilities location
\begin{table}[]
\centering
\caption{Summary of refined GPS \& Galileo servicing depots with $\msdry = 500$ \SI{}{kg} and $D = 1$}
\begin{tabular}{llllllllll}
\hline
\hline
% & \multicolumn{7}{c}%8}{c}
% {$D = 1$} 
% \\  
% \cline{3-9}%-10}
$\mddry$, \SI{}{kg}  & No. &
$a$, \SI{}{DU}   & $e$   & $i$, \SI{}{deg}  & $\Omega$, \SI{}{deg}  & $\mdwet$, \SI{}{kg} & $\Delta \mdwet$, \SI{}{kg} &
\begin{tabular}[c]{@{}l@{}} Reduction \\ of $\mdwet$, \% \end{tabular}
%& 
%EMLEO \SI{}{kg}
\\
\hline
% m = 1500 kg
\multirow{6}{*}{1500}
& 1 & 1.0488 & 0.0325 & 56.98 & 19.39 & 5037 & -978 & -14.09 \\%&  8136 \\
& 2 & 0.5606 & 0.5375 & 54.62 & 90.59 & 2728 &  -30 & -2.89  \\%&  4187 \\
& 3 & 0.5812 & 0.5661 & 54.67 & 139.74 & 4571 & -275 & -6.19 \\%&  7106 \\
& 4 & 0.5110 & 0.4936 & 54.56 & 202.21 & 2461 &  -40 & -3.59 \\%&  3663 \\
& 5 & 0.5571 & 0.5009 & 54.91 & 260.28 & 4579 & -103 & -4.69 \\%&  6976 \\
& 6 & 0.6122 & 0.3192 & 54.72 & 324.97 & 3676 &  -11 & -0.90 \\%&  5552 \\
\hline
% m = 2000 kg
\multirow{5}{*}{2000}
& 1 & 0.9782 & 0.0391 & 56.42 & 19.54 & 5883 & -850 & -11.09 \\%&  9376 \\
& 2 & 0.5382 & 0.5187 & 54.79 & 90.62 & 3278 & -448 & -1.10  \\%&  4966 \\
& 3 & 0.5813 & 0.5661 & 54.77 & 139.79 & 5074 & -286 & -5.85 \\%&  7889 \\
& 4 & 0.6218 & 0.5829 & 51.84 & 243.28 & 7501 &   28 & -0.86 \\%& 11871 \\
& 5 & 0.4831 & 0.4770 & 54.18 & 325.73 & 4306 &  -32 & -1.24 \\%&  6295 \\
\hline
% m = 2500 kg
\multirow{3}{*}{2500} 
& 1 & 0.8762 & 0.5199 & 52.68 & 1.99 & 10781 &   57 & -0.31  \\%& 18116 \\
& 2 & 0.6285 & 0.5871 & 52.42 & 120.60 & 8967 &   24 & -0.67 \\%& 14232 \\
& 3 & 0.6204 & 0.5818 & 51.51 & 243.56 & 8004 &   24 & -0.99 \\%& 12659 \\
\hline
\hline
\end{tabular}
\label{tab:refined_gnss_locations_D1}
\end{table}
